Specification of Products and Product Lines

The study of variability in software development has become increasingly important in recent years. A common mechanism to represent the variability in a product line is by means of feature models. However, the relationship between these models and UML design models is not straightforward. UML statecharts are extended introducing variability in their main components, so that the behavior of product lines can be specified. The contribution of this work is the proposal of a rule-based approach that defines a transformation strategy from extended statecharts to concrete UML statecharts. This is accomplished via the use of feature models, in order to describe the common and variant components, in such a way that, starting from different feature configurations and applying the rule-based method, concrete state machines corresponding to different products of a line can be obtained.

==> eptcsdata.tex <==
\providecommand{\event}{M. Fernandez (Ed.): 9th Int. Workshop on Reduction Strategies\\
in Rewriting and Programming (WRS'09)}
\providecommand{\volume}{15}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{44}
\providecommand{\eid}{4}

